Spectrum and thermodynamic properties of two-dimensional N=(1,1) super Yang-Mills theory with fundamental matter and a Chern-Simons term

We consider N=(1,1) super Yang-Mills theory in 1+1 dimensions with fundamentals at large-N_c. A Chern-Simons term is included to give mass to the adjoint partons. Using the spectrum of the theory, we calculate thermodynamic properties of the system as a function of the temperature and the Yang-Mills coupling. In the large-N_c limit there are two non-communicating sectors, the glueball sector, which we presented previously, and the meson-like sector that we present here. We find that the meson-like sector dominates the thermodynamics. Like the glueball sector, the meson sector has a Hagedorn temperature T_H, and we show that the Hagedorn temperature grows with the coupling. We calculate the temperature and coupling dependence of the free energy for temperatures below T_H. As expected, the free energy for weak coupling and low temperature grows quadratically with the temperature. Also the ratio of the free energies at strong coupling compared to weak coupling, r_{s-w}, for low temperatures grows quadratically with T. In addition, our data suggest that r_{s-w} tends to zero in the continuum limit at low temperatures.

==> tabl0.tex <==
\begin{tabular}{cc}
\hline \hline\\[-4.0mm]
$g$ & $T_{H}^{\infty}$ \\[1mm]
 & $[10^{-4}]$\\[2mm]
\hline\hline\\[-2.5mm]
         0 &       0.52 \\
       0.1 &      0.515 \\
       0.3 &      0.564 \\
       0.5 &       0.69 \\
         1 &       0.86 \\
         2 &      1.564 \\
         3 &      2.259 \\
         4 &       2.88 \\
\hline
\end{tabular}  


==> tabl1.tex <==
\newcommand{\rbx}[1]{\raisebox{-1.5ex}[0pt]{#1}}

%\begin{scriptsize}
\begin{tabular}{ccccc}
\hline \hline\\[-2.0mm]
$T$ & $\tilde{\mathcal{F}}_{spect.}$ & $\tilde{\mathcal{F}}_{fit}$
&$\tilde{\mathcal{F}}^{<}_{fit}$&$\tilde{\mathcal{F}}_{0}$
\\[1.0mm]
$[\kappa]$& $[10^{-2} \kappa^2]$&$[10^{-2} \kappa^2]$&$[10^{-2} \kappa^2]$& $[10^{-2} \kappa^2]$\\[2.0mm]
\hline\hline\\[-0.5mm]
0 & 0 & 0 & 0 &0\\ 
0.025 & 0.00658 & 0.00654 & 0.00654& 0.0009\\ 
0.05 & 0.03459 & 0.03448 & 0.03448 &0.0038\\ 
0.075 & 0.08522 & 0.08499 & 0.08499 &0.0085\\ 
0.1 & 0.15852 & 0.15810 & 0.15809 &0.0151\\ 
$\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ \\ 
0.225 & 0.89782 & 0.89487 & 0.86245 &0.0765\\ 
0.25 & 1.14656 & 1.14269 & 1.07109 &0.0944\\ 
0.275 & 1.44823 & 1.44337 & 1.30232 &0.1142\\ 
0.3 & 1.81661 & 1.81078 & 1.55613 &0.1359\\ 
$\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ \\ 
0.425 & 5.33793 & 5.33113 & 3.16396 &0.2728\\ 
0.45 & 6.54702 & 6.54176 & 3.55327 &0.3059\\ 
0.475 & 7.98870 & 7.98597 & 3.96515 &0.3408\\ 
0.5 & 9.69247 & 9.69351 & 4.39962 &0.3776\\ 
\hline
\end{tabular}
%\end{scriptsize}


==> tabl2b.tex <==
%\begin{scriptsize}
\begin{tabular}{ccccc}
\hline \hline\\[-2.0mm]
$T$ & $\tilde{\mathcal{F}}$ & $\tilde{\mathcal{F}}_{T^+}$
&$\tilde{\mathcal{F}}_{1}$& $\tilde{\mathcal{F}}_{0}$
\\[1.0mm]
$[\kappa]$& $[10^{-2} \kappa^2]$&$[10^{-2} \kappa^2]$&$[10^{-2} \kappa^2]$&$[10^{-2} \kappa^2]$\\[2.0mm]
\hline\hline\\[-0.5mm]
         0 &     0 &     0 &     0 &     0 \\
     0.025 &     0 &     0 &     0 &     0.0008 \\
      0.05 &     0.0002 &     0.0002 &     0.0002 &     0.0033 \\
     0.075 &     0.0011 &     0.0011 &     0.0011 &     0.0074 \\
       0.1 &     0.0033 &     0.0033 &     0.0033 &     0.0131 \\
     $\vdots$ &     $\vdots$ &     $\vdots$ &     $\vdots$ &     $\vdots$ \\
     0.225 &     0.0384 &     0.0383 &     0.0383 &     0.0663 \\
      0.25 &     0.0505 &     0.0503 &     0.0503 &     0.0818 \\
     0.275 &     0.0644 &     0.0641 &     0.0639 &     0.0990 \\
       0.3 &     0.0803 &     0.0796 &     0.0793 &     0.1178 \\
     $\vdots$ &     $\vdots$ &     $\vdots$ &     $\vdots$ &     $\vdots$ \\
     0.425 &     0.1959 &     0.1867 &     0.1813 &     0.2364 \\
      0.45 &     0.2283 &     0.2149 &     0.2068 &     0.2651 \\
     0.475 &     0.2647 &     0.2458 &     0.2340 &     0.2953 \\
       0.5 &     0.3056 &     0.2795 &     0.2628 &     0.3272 \\
\hline
\end{tabular}
%\end{scriptsize}  


==> tabl3b.tex <==
\newcommand{\rbx}[1]{\raisebox{-1.5ex}[0pt]{#1}}

\begin{tabular}{cccc}
\hline\hline \\[-4.0mm]
%\multicolumn{4}{c}{$\mathbf{K=14, \,Z^{+}}$ at $\mathbf{g=0.1}$;
%$\mathbf{M^2 \,\in\, [1.22823,9.10283]\kappa^2}$}\\
%\hline \\[-2.5mm]
%
$\tau$ & $\tilde{\mathcal{F}}_{fit}$ & $\tilde{\mathcal{F}}_{spect.}$
&\rbx{
$\bigl|\frac{\tilde{\mathcal{F}}_{spect.}-\tilde{\mathcal{F}}_{fit}}{\tilde{\mathcal{F}}_{spect.}}\bigr|
\%$}
\\[-1.5mm]
$[\kappa]$& $[10^{-2}\kappa^2]$&$[10^{-2}\kappa^2]$&\\[-0.1mm]
\hline\hline\\[-2.5mm]
0.10 & 0 & 0 & 0 \\
0.125 & 0.00013 & 0.00012 & 7.69 \\
0.15 & 0.00094 & 0.00089 & 5.32 \\
0.175 & 0.00408 & 0.00392 & 3.92 \\
0.20 & 0.01293 & 0.01258 & 2.71 \\
0.225 & 0.03306 & 0.03242 & 1.94 \\
$\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ \\
0.325 & 0.43095 & 0.42919 & 0.41 \\
$\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ \\
0.425 & 2.16541 & 2.16719 & 0.08 \\
0.450 & 2.98414 & 2.98851 & 0.15 \\
0.475 & 4.01281 & 4.02084 & 0.20 \\
\hline
\end{tabular}


==> tabl4REV.tex <==
\newcommand{\rbx}[1]{\raisebox{-1.5ex}[0pt]{#1}}

\begin{tabular}{ccccccccc}
\hline\hline \\[-4.0mm]
%
$T/\kappa$& 0.20 & 0.25 & 0.30 & 0.35 & 0.40 & 0.45 & 0.50 & 0.55\\\hline\hline
%
%
$\tilde{\mathcal{F}}_{meson}/\kappa^2$ & 0.009 & 0.016 & 0.026 & 0.040 & 0.059 & 0.089 & 0.133 & 0.199 \\
%
%
$\tilde{\mathcal{F}}_{glueball}/\kappa^2$ & 0.000 & 0.000 & 0.001 & 0.004 & 0.011 & 0.026 & 0.053 & 0.101 \\
\hline
\end{tabular}


==> tabl5.tex <==
\begin{tabular}{ccccc}
\hline \hline\\[-4.0mm]
$T$ & $r_{s-w}(K=13)$ & $r_{s-w}(K=14)$ & $r_{s-w}(K=15)$ & $r_{s-w}(K=16)$ \\[1mm]
$[\kappa]$& $[10^{-4}]$& $[10^{-4}]$& $[10^{-4}]$& $[10^{-4}]$\\[2mm]
\hline\hline\\[-2.5mm]
      0.025 &       0.12 &       0.19 &       0.29 & 0.50\\
      0.05 &      10.44 &      11.32 &      12.89 &   16.56\\
     0.075 &      42.95 &      41.24 &      42.71 &    49.97\\
       0.1 &      84.74 &      76.62 &      75.77 &    84.72\\
      0.15 &     161.82 &     138.05 &     130.57 &    139.74\\
       0.2 &     217.32 &     180.08 &     166.48 &    174.25\\
       0.3 &     262.02 &     208.95 &     186.77 &    188.81\\
       0.4 &     235.75 &     180.94 &     154.97 &    149.70\\
      0.45 &     207.06 &     155.59 &     129.71 &    121.84\\
       0.5 &     174.62 &     128.31 &     103.76 &    94.57\\
\hline
\end{tabular}


